Attribute Based Administration of Role Based Access Control : A Detailed Description

Administrative Role Based Access Control (ARBAC) models deal with how to manage user-role assignments (URA), permission-role assignments (PRA), and role-role assignments (RRA). A wide variety of approaches has been proposed in the literature for URA, PRA, and RRA. In this paper, we propose attribute-based administrative models that unify many prior approaches for URA and PRA. The motivating factor is that attributes of various RBAC entities such as admin users, regular users and permissions can be used to administer URA and PRA in a highly flexible manner. We develop an attribute-based URA model called AURA and an attribute-based PRA model called ARPA. We demonstrate that AURA and ARPA can express and unify many prior URA and PRA models.

==> source_tex/arpa_save.tex <==

\subsection{ARPA Model}
\label{sec:arpa}
 \input{source_tex/arpa_model}
Administration decisions in ARPA model are based on attributes of
permission and admin user.  ARPA model can be regarded as dual of AURA
model in AARBAC. Table~\ref{tab:arpa} shows sets and functions used in ARPA
model. \AU\ and \R\ are sets of admin users and roles. \RH\ is a
partially ordered roles. There are two operations, {assign} and {revoke}
in set \OP. \P\ is a finite set of permissions. \AATT\ and \PATT\ are
finite sets of admin user attributes and permission attributes,
respectively. We note that attribute names in \AATT\ and \PATT\ are
independent of attribute names in AURA model. \scope(\it{att}) and
attType(\it{att}) are functions determine scope and type of attribute name,
\it{att}. is\_ordered(\it{att}) specifies if attribute values are ordered,
and H\textsubscript{\it{att}} for any attribute name \it{att} in \AATT\ and \PATT\ is
a partial order on attribute values set. 

ARPA has capability to assign a single permission to a role or a set of
permissions to a role.  Authorization functions
{\isauth}P\textsubscript{\it{op}}(\it{au}: \AU, \it{p} : \P, \it{r} : \R) is
designed to assign single user to a role, where operation \it{op} is either
{assign} or {revoke}. This authorization function allows an admin user
\it{au} to assign permission \it{p} to role \it{r} if assignment criteria
is met. This decision is based on the result of logical expression that is
built using attributes of admin user \it{au} and permission \it{p}.  ARPA
also allows an admin user \it{au} to execute operations {assign} or
{revoke} between set of permissions $\chi$ and \it{r} whose function is
given by {\isauth}P\textsubscript{\it{op}}(\it{au}: \AU, $\chi$ : 2\textsuperscript{\P}, \it{r}
: \R). Here, $\chi$  is computed using a set-builder notation, with rules
written using attributes of permission. 

In next section, we will take PRA-Uni model~\cite{BiswasUni} instance and
translate it into an equivalent ARPA instance.  Beside PRA-Uni, we have
successfully mapped instances of following models into equivalent ARPA
instances : PRA97, PRA99, PRA02, and PRA-U. Due to space limitation, these
models are discussed in a full-length document available at
https://arxiv.org. 


